Machine Learning-Based Self-Compensating Approximate Computing

Dedicated hardware accelerators are suitable for parallel computational tasks. Moreover, they have the tendency to accept inexact results. These hardware accelerators are extensively used in image processing and computer vision applications, e.g., to process the dense 3-D maps required for self-driving cars. Such error-tolerant hardware accelerators can be designed approximately for reduced power consumption and/or processing time. However, since for some inputs the output errors may reach unacceptable levels, the main challenge is to \textit{enhance the accuracy} of the results of approximate accelerators and keep the error magnitude within an allowed range. Towards this goal, in this paper, we propose a novel machine learning-based self-compensating approximate accelerators for energy efficient systems. The proposed error \textit{compensation module}, which is integrated within the architecture of approximate hardware accelerators, efficiently reduces the accumulated error at its output. It utilizes \textit{lightweight supervised machine learning techniques, i.e., decision tree}, to capture input dependency of the error. We consider image blending application in multiplication mode to demonstrate a practical application of self-compensating approximate computing. Simulation results show that the proposed design of self-compensating approximate accelerator can achieve about 9\% accuracy enhancement, with negligible overhead in other performance measures, i.e., power, area, delay and energy.

==> Extra.tex <==
Array multipliers are not the fastest neither the smallest multipliers. However, their periodic structure has a compact hardware layout, thanks
to short wiring, and allows for efficient pipelining. This advantage makes array multiplier one of the most used in embedded System on Chip (SoC).


Autonomous systems (ASs) can respond to real world conditions automatically without human intervention. It is often based on artificial intelligence because machine learning techniques are used to model the complex real world. For example, self-driving cars rely on global positioning system (GPS) sensing knowledge to help with navigation, sensors to avoid collisions and augmented reality to displays information to drivers in innovative ways.

the US Department of Transportation's National Highway Traffic Safety Administration (NHTSA) has formally defined five different levels of autonomous driving  \cite{CAAD}

Autonomous vehicles sense their surroundings by multiple sensors and cameras. Therefore, it places an extremely high demands in terms of computation speed and power consumption to be able to process the enormous amount of sensors data.


Systems Architecture 

A system architecture can consist of system components and the sub-systems developed, that will work together to implement the overall system.


A modern automobile runs vastly more software than the Apollo spacecraft
